GenAIPABench: A Benchmark for Generative AI-based Privacy Assistants

Privacy policies of websites are often lengthy and intricate. Privacy assistants assist in simplifying policies and making them more accessible and user friendly. The emergence of generative AI (genAI) offers new opportunities to build privacy assistants that can answer users questions about privacy policies. However, genAIs reliability is a concern due to its potential for producing inaccurate information. This study introduces GenAIPABench, a benchmark for evaluating Generative AI-based Privacy Assistants (GenAIPAs). GenAIPABench includes: 1) A set of questions about privacy policies and data protection regulations, with annotated answers for various organizations and regulations; 2) Metrics to assess the accuracy, relevance, and consistency of responses; and 3) A tool for generating prompts to introduce privacy documents and varied privacy questions to test system robustness. We evaluated three leading genAI systems ChatGPT-4, Bard, and Bing AI using GenAIPABench to gauge their effectiveness as GenAIPAs. Our results demonstrate significant promise in genAI capabilities in the privacy domain while also highlighting challenges in managing complex queries, ensuring consistency, and verifying source accuracy.

==> abstract.tex <==

% Privacy policies inform users about the data management practices of organizations. Yet, their complexity often renders them largely incomprehensible to the average user, necessitating the development of \textit{privacy assistants}. With the advent of generative AI (genAI) technologies, there is an untapped potential to enhance privacy assistants in answering user queries effectively. However, the reliability of genAI remains a concern due to its propensity for generating incorrect or misleading information. This study introduces \benchmark, a novel benchmarking framework designed to evaluate the performance of Generative AI-based Privacy Assistants (GenAIPAs). \benchmark comprises: 1) A comprehensive set of questions about an organization's privacy policy and a data protection regulation, along with annotated answers for several organizations and regulations; 2) A robust set of evaluation metrics for assessing the accuracy, relevance, and consistency of the generated responses; and 3) An evaluation tool that generates appropriate prompts to introduce the system to the privacy document and different variations of the privacy questions to evaluate its robustness. We use \benchmark to assess the potential of three leading genAI systems in becoming GenAIPAs —ChatGPT, Bard, and Bing AI. Our results demonstrate significant promise in genAI capabilities in the privacy domain while also highlighting challenges in managing complex queries, ensuring consistency, and verifying source accuracy.
% % Our findings set the stage for future enhancements in the field of privacy assistant technologies.
Privacy policies of websites are often lengthy and intricate. \textit{Privacy assistants} assist in simplifying policies and making them more accessible and user-friendly. The emergence of generative AI (genAI) offers new opportunities to build privacy assistants that can answer users' questions about privacy policies. However, genAI's reliability is a concern due to its potential for producing inaccurate information. This study introduces \benchmark, a benchmark for evaluating Generative AI-based Privacy Assistants (GenAIPAs). \benchmark includes: 1) A set of questions about privacy policies and data protection regulations, with annotated answers for various organizations and regulations; 2) Metrics to assess the accuracy, relevance, and consistency of responses; and 3) A tool for generating prompts to introduce privacy documents and varied privacy questions to test system robustness. We evaluated three leading genAI systems—ChatGPT-4, Bard, and Bing AI—using \benchmark to gauge their effectiveness as GenAIPAs. Our results demonstrate significant promise in genAI capabilities in the privacy domain while also highlighting challenges in managing complex queries, ensuring consistency, and verifying source accuracy.

==> methodology.tex <==
\begin{algorithm}[tbh]
\caption{GenAIPA Response and Summary Generation } 
\label{alg:response_generation_evaluation2}
\begin{algorithmic}[1]
\Procedure{GenAndEvalResp}{Privacy Document PD, Questions Q, Runs r}
\State \textbf{Step 1: Response Generation}
\State $A \gets \emptyset$
\For{$i=1$ to $r$}
\State $A_i \gets \emptyset$
\State IntroducePrivacyDocument(PD)
\State $Q' \gets \text{ShuffleQuestions}(Q)$
\For{each $q$ in $Q'$}
\State $A_i \gets \text{SendQuestion}(q)$
\State $A \gets \{q, A_i\}$
\EndFor
\EndFor
\State \textbf{Step 2: Summary Generation}
\State $C \gets \text{SplitPolicy}(PD)$
\State Initialize empty list $D$
\For{$c \in C$}
\State $d \gets \text{Prompt}(c)$
\State Add $d$ to $D$
\EndFor
\State $S \gets \text{GenerateSummary}(D)$
\State Return $S$
\end{algorithmic}
\label{Algorithm2}
\end{algorithm}


The \benchmark includes a component evaluator whose goal is to communicate with the GenAIPA, sharing the privacy documents and questions and collecting answers and summaries (see Algorithm \ref{alg:response_generation_evaluation2}). This is accomplished in a two-step process: response generation (see Step 1 of Algorithm \ref{alg:response_generation_evaluation2}) and summary generation (See Step 2 of Algorithm \ref{alg:response_generation_evaluation2}). In the response generation stage, an evaluator has two ways to introduce GenAIPA to the privacy document. In the first instance,  the privacy document is partitioned into smaller sections, accommodating the input capacity of GenAIPA. Simultaneously, an empty list intended for holding conversation sets is initialized. Next, a new conversation is initiated.  After initiating a conversation with GenAIPA, the policy sections are systematically introduced to the GenAIPA. For every initiated conversation, the question list is shuffled, and each question within this reordered list is utilized as a prompt for the GenAIPA. The responses to each question are collected, organized into question-answer pairs, and added to their respective conversation sets. This entire procedure is repeated thrice for each privacy policy, resulting in a collection of three distinct conversation sets per policy. In the second instance, the privacy policy corpus is leveraged to ascertain whether the GenAIPA model was trained on a previous version of these policies. Using the evaluator, queries are then directed to GenAIPA to
verify the version and date of the privacy policy with which it is familiar, assuming the system has access to the given
policy. GenAIPA is thus requested to disclose the version and date of the privacy policy it last accessed. The disclosed
version and date are subsequently used as a reference to retrieve the identical version of the privacy policy via the
 \textit{Wayback Machine}\footnote{\url{https://archive.org/web/}}, an online digital archive that allows access to historical versions of internet content. This retrieved
version serves as the gold standard in our analysis, providing accurate answers to the privacy questions that will be later
asked to the GenAIPA. 
The ensuing step involves prompting GenAIPA with questions about the privacy policy,
using the evaluator, which resembles step 1 of Algorithm\ref{alg:response_generation_evaluation2} to generate responses. The final phase of the procedure involves the evaluator comparing the GenAIPA responses with the annotated answers that were previously identified by analysts through the detailed examination of the retrieved policies from the
Wayback Machine. 

In the summary generation step, the procedure begins by Utilizing the evaluator to query GenAIPA to craft a succinct summary of the privacy policy (see Algorithm \ref{alg:policy_evaluation3}). This involves creating an efficient summary by feeding segments of the policy to GenAIPA. The evaluator initiates the process by partitioning the input policy into several segments, each supplied to GenAIPA individually. After all segments have been processed, GenAIPA is queried to create a thorough summary. This synthesized summary is then utilized as the input for the ensuing stage. Once the summary is generated, the evaluator uses it as input for GenAIPA. Subsequently, our curated set of privacy-related questions (see Section \ref{sect:questions}) are posed as prompts by the evaluator to GenAIPA to assess the depth and accuracy of the information contained in the summary. In response, GenAIPA crafts answers based on the summary. This procedure aligns with the response generation of the evaluator tool. For every question, the evaluator generates three different responses and evaluates the quality of the information derived from the summary using the response evaluation (see Algorithm\ref{alg:response_generation_evaluation2}).








% the privacy policy corpus is leveraged to ascertain whether the GenAIPA model
% was trained on a previous version of these policies. Using the evaluator, queries are then directed to GenAIPA to
% verify the version and date of the privacy policy with which it is familiar, assuming the system has access to the given
% policy. GenAIPA is thus requested to disclose the version and date of the privacy policy it last accessed. The disclosed
% version and date are subsequently used as a reference to retrieve the identical version of the privacy policy via the
%  \textit{Wayback Machine}\footnote{\url{https://archive.org/web/}}, an online digital archive that allows access to historical versions of internet content. This retrieved
% version serves as the gold standard in our analysis, providing accurate answers to the privacy questions that will be later
% asked to the GenAIPA. 
% The ensuing step involves prompting GenAIPA with questions related to the privacy policy,
% using the evaluator which resembles step 1 of Algorithm\ref{alg:response_generation_evaluation2} to generate responses. The final phase of the experiment involves the evaluator comparing the GenAIPA responses with
% the correct answers that were previously identified through the detailed examination of the retrieved policies from the
% Wayback Machine. 

 

% In Step 1, the given privacy policy is partitioned into smaller sections to accommodate the constraints of ChatGPT's input capacity (3000 words). Simultaneously, an empty list intended for holding conversation sets is initialized. Next, a new ChatGPT conversation is initiated. Each part of the partitioned privacy policy is systematically introduced to ChatGPT. For every initiated conversation, the question list is shuffled, and each question within this reordered list is utilized as a prompt for ChatGPT. Subsequently, the answers to each question are collected and organized into question-answer pairs. These pairs are then appended to the respective conversation set. This procedure is repeated thrice for each privacy policy. The outcome is a collection of three distinct conversation sets per privacy policy. In Step 2, we analyze the generated responses based on predefined metrics and evaluation scheme (see Section\ref{sect:metrics}). We repeat this process for each conversation set and store the average normalized scores for each run. Finally, we calculate the overall average normalized score across the three runs. By applying this two-step AI response evaluation algorithm (Algorithm \ref{alg:response_generation_evaluation2}), we aim to assess the performance of ChatGPT in generating privacy policy-related responses, identify areas for improvement, and understand the reliability of ChatGPT in the context of privacy policies.


%To investigate the language generation capabilities of ChatGPT, we conducted an analysis using the two-step AI response generation and evaluation algorithm (Algorithm \ref{alg:response_generation_evaluation2}) to determine whether the model generates the same or different responses to the same question when presented with paraphrased versions of the question. This analysis is crucial because it provides insights into the diversity and quality of the model's language generation capabilities, which are essential for various applications. To conduct this analysis, we first generated  paraphrased versions of the same questions. We used publicly available paraphrasing tools like quillbot\cite{quillbot} to ensure that the paraphrased questions were semantically equivalent to the original question. Next, we input each of the paraphrased questions into the AI response generation and evaluation algorithm's response generation step (Step 1) and recorded the responses provided by ChatGPT. Finally, we analyzed the generated responses using the AI response evaluation step (Step 2) of the algorithm and compared the responses generated by ChatGPT for each of the paraphrased questions to determine whether the model provided the same or different responses. The results of this analysis provide valuable insights into the language generation capabilities of ChatGPT and can be used to evaluate the suitability of the model for various applications when combined with the two-step AI response generation and evaluation algorithm (Algorithm \ref{alg:response_generation_evaluation2}).

% To gauge ChatGPT's ability to provide similar responses to a question and its paraphrased version, we carried out a robustness analysis. We used Algorithm \ref{alg:response_generation_evaluation2} to check if the model gives the correct answers when presented with a paraphrased form of a question. This analysis is vital as it tests ChatGPT's consistency in generating responses to varied forms of the same question, fostering clear communication and improving user experience. To conduct this analysis, we first generated paraphrased versions of our sample corpus (see Section \ref{sect:questions}) by using publicly available paraphrasing tools like QuillBot\cite{quillbot}, which uses ML algorithms to ensure that the paraphrased questions (see Table \ref{ques:T3}) were semantically equivalent to the original question. Next, we apply the identical methodology as used in the preceding analysis, where  the variations were then used to test ChatGPT's comprehension and answer-generation abilities. The primary divergence in this stage was the introduction of paraphrased questions, rather than benchmark queries, as the basis for response generation. Finally, we analyzed the generated responses using (Step 2) of the Algorithm\ref{alg:response_generation_evaluation2} and evaluated the responses with the metrics (see Section \ref{sect:metrics}).  By testing the model on a variety of question variations, we can assess its ability to generalize and understand the intent behind the questions, even if they are phrased in different ways. This is critical for building effective natural language processing models, especially in the context of privacy policies where the language can be complex and difficult to understand.


%\subsubsection{Assessing ChatGPT's Performance in Privacy Policy Analysis}

% \subsection{Assessing Privacy Policy Adherence of ChatGPT}
% In this study, our primary goal is to assess the proficiency of ChatGPT in producing responses related to the specific version of the privacy policy it was trained on. We begin the procedure by identifying a product that has a publicly available privacy policy. Following this, we query ChatGPT to ascertain the version and date of the product's privacy policy it has knowledge of. In instances where the ChatGPT has access to the policy, we request the model to furnish us with the version and the date it was accessed. Utilizing this version and date as a reference, we subsequently interact with the \textit{Wayback Machine} \footnote{\url{https://archive.org/web/}} to retrieve the identical version for comparison purposes. The next step involves, prompting ChatGPT with privacy questions (See section \ref{sect:questions} ), stimulating it to generate responses (See step 1) of Algorithm \ref{alg:response_generation_evaluation2}. The distinguishing feature of this study is that, unlike our previous approach, we do not feed any privacy policy information to ChatGPT. This adjusted methodology enables us to assess the inherent capability of ChatGPT to recall and apply privacy policy information without explicit external input. The responses generated by ChatGPT undergo the same evaluation process as defined in Section  \ref{sect:metrics}, adhering to the established assessment criteria used in our previous analysis.
% By leveraging this comprehensive and systematic approach, we can assess the inherent capacity of ChatGPT to recall and apply privacy policy knowledge accurately, thereby providing valuable insights into the model's proficiency and limitations in handling real-world privacy-related inquiries.


% \subsection{Assessing the Ability to Recall Learned Privacy Policy Knowledge}




% In the initial phase of the experiment, the privacy policy corpus is leveraged to ascertain whether the GenAIPA model was trained on a previous version of these policies. Using an evaluator tool, queries are then directed to GenAIPA to verify the version and date of the privacy policy with which it is familiar, assuming the system has access to the given policy. GenAIPA is thus requested to disclose the version and date of the privacy policy it last accessed.
% The disclosed version and date are subsequently used as a reference to retrieve the identical version of the privacy policy via the \textit{Wayback Machine}\footnote{\url{https://archive.org/web/}}, an online digital archive that allows access to historical versions of internet content. This retrieved version serves as the gold standard in our analysis, providing accurate answers to the privacy questions that will be later asked to the GenAIPA.
% The ensuing step involves prompting GenAIPA with questions related to the privacy policy, using the evaluator tool. This task stimulates the GenAIPA to generate responses based on its previously acquired knowledge.
% The final phase of the experiment involves the evaluator tool comparing the GenAIPA responses with the correct answers that were previously identified through the detailed examination of the retrieved policies from the Wayback Machine.
% Notably, this study deviates from our previous methodologies in that it does not involve feeding any privacy policy information to the GenAIPA. This approach allows for an evaluation of GenAIPAs inherent capacity to recall and apply privacy policy knowledge without the need for explicit external input. The evaluator tool is used to analyze the responses generated by GenAIPA, following the same evaluation process as in the previous studies.
% By observing the consistency of responses and the ability to recall specific details, this research seeks to provide insights into the extent of GenAIPAs retention and application of privacy policy knowledge. This, in turn, could have significant implications for future applications and training processes of GenAIPA, particularly in areas where adherence to specific privacy principles is paramount.


% \begin{algorithm}[H]
% \caption{ChatGPT Response Generation and Evaluation}\label{alg:response_generation_evaluation2}
% \begin{algorithmic}[1]
% \Procedure{GenAndEvalResp}{Questions Q}
% \State \textbf{Step 1: Response Generation}
% \State Initialize empty set of Conversations $A$
% \For{$i=1$ to $3$}
% \State $Q_i \gets \text{ShuffleQuestions}(Q)$
% \State Initialize empty set of Conversation $C_i$
% \For{each question $q$ in $Q_i$}
% \State $answer \gets \text{SendPrompt}(q)$
% \State Add $q$ and $answer$ to Conversation $C_i$
% \EndFor
% \State Add Conversation $C_i$ to Set of Conversations $A$
% \EndFor

% \State \textbf{Step 2: ChatGPT Response Evaluation}
% \State Initialize empty list $S$
% \For{$A_i \in A$}
% \State Initialize scores for $M_{rel}, M_{acc}, M_{cla}, M_{com}, M_{ref}$ to 0
% \For{$f \in {M_{rel}, M_{acc}, M_{cla}, M_{com}, M_{ref}}$}
% \State Evaluate $f$
% \EndFor
% \State Calculate total points for each feature
% \State Normalize scores and store them for $A_i$
% \State Add average normalized score for $A_i$ to $S$
% \EndFor
% \State Calculate overall avg. score in $S$
% \State Categorize response: Green, Yellow, Red
% \State \textbf{return} Category
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}



% \subsection{Assessing the Quality of Privacy Policy Summaries Generated by genAI System} 


% \begin{algorithm}[H]
% \caption{Response Generation and Evaluation}\label{alg:policy_evaluation3}
% \begin{algorithmic}[1]
% \Procedure{EvaluatePolicy}{Policy P, Questions Q}
% \State \textbf{Step 1: Summary Generation}
% \State $C \gets \text{SplitPolicy}(P)$
% \State Initialize empty list $D$
% \For{$c \in C$}
% \State $d \gets \text{Prompt}(c)$
% \State Add $d$ to $D$
% \EndFor
% \State $S \gets \text{Summarize}(D)$

% \State \textbf{Step 2: ChatGPT Response Generation}
% \State Initialize empty list $A$
% \For{$i=1$ to $3$}
% \State Open ChatGPT window
% \State Initialize empty set $A_i$
% \State $Q' \gets \text{Shuffle}(Q)$
% \For{$q \in Q'$}
% \State $a \gets \text{Prompt}(S, q)$
% \State Add $q, a$ to $A_i$
% \EndFor
% \State Add $A_i$ to $A$
% \EndFor

% \State \textbf{Step 3: ChatGPT Response Evaluation}
% \State Initialize empty list $S$
% \For{$A_i \in A$}
% \State Initialize scores for $M_{rel}, M_{acc}, M_{cla}, M_{com}, M_{ref}$ to 0
% \For{$f \in {M_{rel}, M_{acc}, M_{cla}, M_{com}, M_{ref}}$}
% \State Evaluate $f$
% \EndFor
% \State Calculate total points for each feature
% \State Normalize scores and store them for $A_i$
% \State Add average normalized score for $A_i$ to $S$
% \EndFor
% \State Calculate overall avg. score in $S$
% \State Categorize response: Green, Yellow, Red
% \State \textbf{return} Category
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}


\begin{algorithm}[H]
\caption{GenAIPA Response Evaluation}\label{alg:policy_evaluation3}
\begin{algorithmic}[1]
\Procedure{EvaluateResponse}{Scores S provided by analyst}
\State $P \gets \emptyset$
\For{$i = 1$ to $|S[1]|$} 
\State $\overline{S_i} \gets \frac{1}{|S|} \sum_{score \in S} score[i]$
\State Categorize $\overline{S_i}$ as Green, Yellow, or Red
\State $P \gets P \cup {\text{Category}}$
\EndFor
\State \textbf{return} $P$
\end{algorithmic}
\end{algorithm}
In the GenAIPA Response Evaluation process (see Algorithm \ref{alg:policy_evaluation3}), the analyst scrutinizes the generated responses based on five key features: Relevance, Accuracy, Clarity, Completeness, and Reference to policy sections. Scores for each feature are provided as input $S$. The procedure starts by initializing an empty set $P$ and then iterates through each score $S_i$ in $S$, accumulating them for subsequent categorization. This evaluation is performed for each set of scores, representing multiple runs, and the average scores for each run are determined. Ultimately, an overall average score is calculated across all runs. This average score is then categorized into one of three groups: Green, Yellow, or Red, based on predefined criteria (see Section \ref{sect:metrics}. The category is stored in set P, which, upon completion of all iterations, contains the categorized average scores for all runs. The primary goal of this evaluation is to offer insights into GenAIPA's capabilities in generating privacy policy-related responses and identify areas of potential improvement.


% The next aspect of the study is to determine how well the GenAIPA can produce privacy policy summaries that are both user-friendly and comprehensive, thus preserving the critical details of the policies.  The process begins by using the synthesized summary as input for the ensuing stage. 
% This synthesized summary serves as the GenAIPA input, provided by the evaluator. Subsequently, our curated set of privacy-related questions, (see Section \ref{sect:questions}) are posed
% as prompts by the evaluator to GenAIPA in order to assess the depth and accuracy of the information contained in
% the summary. In response, GenAIPA crafts answers based on the summary. This procedure aligns with the response
% generation (see Step 1 of Algorithm \ref{alg:response_generation_evaluation2}) of the evaluator tool. For every question, the evaluator generates three different responses and evaluates the
% quality of the information derived from the summary by using the response evaluation (see Step 2 of Algorithm \ref{alg:response_generation_evaluation2}).
% Through this process, we can evaluate not only the accuracy of the condensed privacy policy summaries but also their practicality. We can ensure that the essential information is retained in the summary and is presented in a manner that users can easily comprehend.


% AI response generation and evaluation algorithm\ref{alg:response_generation_evaluation2}. The process can be segmented into three principal steps:
% \begin{enumerate}
%     \item 

% Utilize ChatGPT to craft a succinct summary of the privacy policy (see Algorithm \ref{Algorithm2}). This involves creating an efficient summary by feeding segments of the policy to ChatGPT. The algorithm initiates by partitioning the input policy into several segments, each supplied to ChatGPT individually. After all, segments have been processed, ChatGPT creates a thorough summary. This synthesized summary is then utilized as the input for the ensuing stage.


% \item
% Once the summary is generated, it is used as input for ChatGPT. Subsequently, our curated set of privacy-related questions, referenced in Section \ref{sect:questions}, are posed as prompts to ChatGPT in order to assess the depth and accuracy of the information contained in the summary. In response, ChatGPT crafts answers based on the summary. This procedure aligns with (Step 1) of our response generation and evaluation algorithm (see Algorithm \ref{alg:response_generation_evaluation2}).
% \item
% For every question, we generate three different responses and evaluate the quality of the information derived from the summary (refer to Step 2 in Algorithm \ref{alg:response_generation_evaluation2}).
% \end{enumerate}.
% This method allows us to evaluate not only the accuracy but also the practicality of a privacy policy summary. It ensures that the condensed summary carries the most crucial information, presented in a clear and comprehensible manner.

% The aim of this study is to evaluate the ability of genAI system to summarize complex privacy policies into more digestible formats. The study seeks to answer the following question: 1)
% Can genAI produce privacy policy summaries that are both user-friendly and comprehensive, preserving the crucial details of the policies?
% The objective is to ensure that genAI retains all vital elements of the policy when condensing it, thus keeping the user fully informed.

% The procedure begins by Utilizing the evaluator tool to query genAI to craft a succinct summary of the privacy policy (see Algorithm \ref{Algorithm2}). This involves creating an efficient summary by feeding segments of the policy to genAI system. The evaluator initiates the process by partitioning the input policy into several segments, each supplied to genAI system individually. After all, segments have been processed, genAI system is queried to create a thorough summary. This synthesized summary is then utilized as the input for the ensuing stage.
% Once the summary is generated, it is used as input for genAI by the evaluator. Subsequently, our curated set of privacy-related questions, (see Section \ref{sect:questions}), are posed as prompts by the evaluator to genAI system in order to assess the depth and accuracy of the information contained in the summary. In response, genAI system crafts answers based on the summary. This procedure aligns with the response generation of the evaluator tool. For every question, the evaluator generates three different responses and evaluates the quality of the information derived from the summary by using the response evaluation.

% This process allows for the evaluation of not only the accuracy of the condensed privacy policy summaries but also their practicality, ensuring that the essential information is retained in the summary and is presented in an easily comprehensible manner.


% \subsection{Assessing the Complexity of Privacy Policy Summaries Generated by genAI System}
% % The assessment of readability in privacy policies is an essential aspect of ensuring that users are capable of understanding the data practices of a product \cite{boerman2018}. To address this issue, we propose a methodology that employs ChatGPT, a language model based on the GPT-3.5 architecture, to generate a summary or simplified version of a privacy policy \cite{brown2020}. After the summary or simplified version is generated, we utilize well-established metrics, such as the Flesch-Kincaid Grade Level and the Gunning Fog Index, to assess its readability \cite{kincaid1975, gunning1952}. These metrics provide a quantitative measure of the complexity of the text, where higher scores indicate more difficult reading levels. By employing these metrics, we can determine the readability of the privacy policy and identify any potential issues with its complexity or length. Complex or lengthy privacy policies can be challenging for users to comprehend, resulting in a lack of informed consent or confusion over the data practices of a product \cite{smith2019}.
% The assessment of readability in privacy policies is an essential aspect of ensuring that users are capable of understanding the data practices of a product \cite{boerman2018}.
% The aim of this study is to evaluate the complexity of the summaries generated by genAI in the context of privacy policies. The purpose is to understand whether the complexity level of these summaries can potentially impact user comprehension. In essence, this study answers the question: 1)
% How complex are the summaries generated by ChatGPT for privacy policies, and does this complexity level affect user comprehension?

% In this study, we first use an evaluator tool to query genAI system to create a summary of the privacy policy (see Subsection 6.5). We then preprocess the summary and privacy policy using the Natural Language Toolkit \textit{(NLTK)}\cite{bird2009natural} to ensure uniformity and clarity. Steps involve breaking the text into sentences, converting words to lowercase, removing stopwords, and reducing words to their base form. Next, we assess the readability using the Textstat \footnote{\url{https://pypi.org/project/textstat/}} library, which uses the Flesch-Kincaid and Gunning-Fog metrics\cite{kincaid1975,gunning1952} to measure text complexity. 
